Lattice Study on quantum-mechanical dynamics of two-color QCD with six light flavors

We investigate the chiral properties of SU(2) gauge theory with six flavors, i.e. six light Dirac fermions in the fundamental representations by lattice simulation, and point out that the spontaneous breakdown of chiral symmetry does not occur in this system. The quark mass dependence of the mesonic spectrum provides an evidence for such a possibility. The decay constant tends to be increased by the finite size effect, which is opposite to the behavior predicted by chiral perturbation theory and indicates that the long distance dynamics in the six-flavor theory could be different from the theory with chiral symmetry breaking. The subtracted chiral condensate, whose utility is demonstrated by the simulation of two-flavor theory, is shown to vanish in the chiral limit within the precision of available data.

==> Table/NF2/tab.NF2.ratios.L16.b2.0.tex <==
\begin{table}[htb]
\caption{Various secondary quantities 
 in two-flavor theory on $L/a=16$ and $\beta = 2.0$ lattices.}
\label{tab:NF2.ratios.L16.b2.0}
\begin{tabular}{cccc}
  \hline
  \hline
  $\kappa$ & $M_V /M_P$ & $f_P /M_P$ & $B \times 10^{-2}$ \\
  \hline
  $0.1540$ & $1.0550\ (24)$  & %$0.2241\  (63)$ & $0.1273\  (72)$\\
   $0.2175\ (30)$ & $0.1346\  (39)$\\

  $0.1580$ & $1.0922\ (29)$  & %$0.2216\  (76)$ & $0.1392\  (96)$\\
   $0.2239\ (29)$ & $0.1363\  (36)$\\

  $0.1620$ & $1.219\ (25)$ & %$0.2570\ (234)$ & $0.1160\ (203)$\\
   $0.2505\ (95)$ & $0.122\ (11)$\\

  $0.1625$ & $1.2329\ (86)$  & %$0.2520\ (189)$ & $0.1236\ (184)$\\
   $0.2543\ (40)$ & $0.1208\ (42)$\\
  $0.1630$ & $1.2905\ (16)$ & %$0.2521\ (205)$ & $0.1254\ (217)$\\
   $0.2608\ (48)$ & $0.1171\ (48)$\\
\hline
\hline
\end{tabular}
\end{table}


==> Table/NF2/tab.NF2.ratios.L16.b4.0.tex <==
\begin{table}[htb]
\caption{Various secondary quantities
 in two-flavor theory on $L/a=16$ and $\beta = 4.0$ lattices.}
\label{tab:NF2.ratios.L16.b4.0}
\begin{tabular}{cccc}
\hline
\hline
$\kappa$ & $M_V /M_P$ & $f_P /M_P$ & $B \times 10^{-2}$ \\
\hline
  $0.1280$ & $1.0064\ (13)$ & %$0.0894\ (13)$ & $1.186\  (38)$\\
   $0.0898\ (11)$ & $1.177\ (35)$\\

  $0.1320$ & $-$            & %$0.0618\ (12)$ & $1.061\  (41)$\\
   $0.06015\  (44)$ & $1.115\ (24)$\\

  $0.1340$ & $1.0182\  (8)$ & %$0.0251\  (9)$ & $2.382\ (168)$\\
   $0.02590\  (20)$ & $2.235\ (41)$\\
\hline
\hline
\end{tabular}
\end{table}


==> Table/NF2/tab.NF2.ratios.L24.b2.0.tex <==
\begin{table}[htb]
\caption{Various secondary quantities 
 in two-flavor theory on $L/a=24$ and $\beta = 2.0$ lattices.}
\label{tab:NF2.ratios.L24.b2.0}
\begin{tabular}{cccc}
\hline
\hline
$\kappa$ & $M_V /M_P$ & $f_P /M_P$ & $B \times 10^{-2}$ \\
\hline
  $0.1540$ & $1.0516\ (29)$ & %$0.2189\ (108)$ & $0.1330\ (127)$\\
  $0.2201\ (17)$ & $0.1315\ (23)$\\

  $0.1620$ & $1.1924\ (63)$ & %$0.2575\ (80)$ & $0.1142\  (70)$  \\
  $0.2570\ (39)$ & $0.1146\ (36)$  \\

  $0.1625$ & $1.2228\ (72)$ & %$0.2530\ (138)$ & $0.1237\ (138)$\\
  $0.2612\ (26)$ & $0.1160\ (15)$\\

  $0.1630$ & $1.2641\ (76)$ & %$0.2612\ (203)$ & $0.1171\ (177)$\\
  $0.2665\ (32)$ & $0.1124\ (24)$\\

  $0.1637$ & $1.404\ (17)$ &
  $0.2888\ (38)$ & $0.1023\ (23)$\\
\hline
\hline
\end{tabular}
\end{table}


==> Table/NF2/tab.NF2.ratios.L24.b4.0.tex <==
\begin{table}[htb]
\caption{Various secondary quantities 
 in two-flavor theory on $L/a=24$ and $\beta = 2.0$ lattices.}
\label{tab:NF2.ratios.L24.b2.0}
\begin{tabular}{cccc}
\hline
\hline
$\kappa$ & $M_V /M_P$ & $f_P /M_P$ & $B \times 10^{-2}$ \\
\hline

$0.1320$ & $1.0247\ (53)$ & %$0.1132\ (12)$ & $1.091\ (19)$\\
 $0.11143\ (79)$ & $1.125\ (12)$\\

$0.1340$ & $-$ & %$0.05822\ (98)$ & $1.879\ (48)$\\
 $0.05818\ (93)$ & $1.881\ (35)$\\

\hline
\hline
\end{tabular}
\end{table}


==> Table/NF6/Stock/tab.NF6.conds.quadratic.b2.0.tex <==
\begin{table}[thb]
\caption{Result for the fit to the chiral condensate by the quadratic fit,
where $b_0$ is the value in chiral limit.} 
\label{tab:NF6.conds.quadratic.b2.0}
\begin{tabular}{cccc}
\hline
\hline
 data set & $b_0$ & $b_1$ & $b_2$ \\ 
\hline
 {\bf S1} & $-0.00003\ (12)$ & $2.4030\ (35)$ & $-0.927\ (21)$\\
 {\bf S2} & $ 0.00017\ (20)$ & $2.3897\ (97)$ & $-0.76\ (10)$\\
 {\bf S3} & $ 0.00142\ (76)$ & $2.382\ (13)$ & $-0.849\ (53)$ \\
\hline
\hline
\end{tabular}
\end{table}

